Optimization and parallelization of B-spline based orbital evaluations in QMC on multi/many-core shared memory processors

B-spline based orbital representations are widely used in Quantum Monte Carlo (QMC) simulations of solids, historically taking as much as 50% of the total run time. Random accesses to a large four-dimensional array make it challenging to efficiently utilize caches and wide vector units of modern CPUs. We present node-level optimizations of B-spline evaluations on multi/many-core shared memory processors. To increase SIMD efficiency and bandwidth utilization, we first apply data layout transformation from array-of-structures to structure-of-arrays (SoA). Then by blocking SoA objects, we optimize cache reuse and get sustained throughput for a range of problem sizes. We implement efficient nested threading in B-spline orbital evaluation kernels, paving the way towards enabling strong scaling of QMC simulations. These optimizations are portable on four distinct cache-coherent architectures and result in up to 5.6x performance enhancements on Intel Xeon Phi processor 7250P (KNL), 5.7x on Intel Xeon Phi coprocessor 7120P, 10x on an Intel Xeon processor E5v4 CPU and 9.5x on BlueGene/Q processor. Our nested threading implementation shows nearly ideal parallel efficiency on KNL up to 16 threads. We employ roofline performance analysis to model the impacts of our optimizations. This work combined with our current efforts of optimizing other QMC kernels, result in greater than 4.5x speedup of miniQMC on KNL.

==> qmcintro.tex <==
\section{QMC and B-spline evaluations}

In quantum mechanics, all physically observable
quantities for a system containing $N_{el}$ particles can be computed from
the $3N_{el}$-dimensional {\em wave function},
$\Psi(\mathbf{r}_1,\dots,\mathbf{r}_{N_{el}})$.  
For any trial {\em wave function}, $\Psi_T(\mathbf{R})$, we can compute an energy as the expectation value of
the many-body Hamiltonian, $\hat{H}$, 
\begin{equation} E_T =
\frac{\int d^{3N}\mathbf{R} \ \Psi_T^*(\mathbf{R}) \hat{H}
\Psi_T(\mathbf{R})} {\int d^{3N}\mathbf{R} \ \left|\Psi_T(\mathbf{R})\right|^2}
\label{eq:Etrial}, 
\end{equation} 
where $\mathbf{R}$ is a $3N$-dimensional vector representing the positions of
the $N$ particles.  A {\em variational principle} guarantees that $E_T \ge E_0$
for all $\Psi_T$, which implies that the lower the energy a given $\Psi_T$ has,
the closer it is to $E_0$, the exact solution of the Schr\"{o}dinger equation. 

The direct evaluation of many-dimensional integrals of Eq.~(\ref{eq:Etrial}) by
stochastic sampling enables us to employ highly accurate variational wave
functions which can capture crucial many-body effects in an efficient manner. 
%The computational effort of QMC is dominated by that of the wave functions.
The Slater-Jastrow trial wave functions, commonly used
in QMC applications to electronic structure, are sums of Slater determinants of
single-particle orbitals multiplied by a Jastrow factor:
\begin{equation}
\Psi_T= \exp (J_1)\exp(J_2) \cdots \sum C_k D_k^{\uparrow} (\{\phi\}) D_k^{\downarrow} (\{\phi\}),
\label{eq:sj}
\end{equation}
%\begin{equation}
%\Psi_T= \exp (J_1)\exp(J_2) \cdots D{\uparrow} (\{\phi\}) D^{\downarrow} (\{\phi\})
%\label{eq:sj}
%\end{equation}
with $N_{el}=N^{\uparrow}+N^{\downarrow}$ for $\uparrow\downarrow$ spins.
For the rest of the paper, we assume  $N_{el}=2N$,
$D^{\downarrow}=D^{\uparrow}$ and $C_0=1$ and zero otherwise.
Here, $\{\phi\}$ denotes a set of SPOs and
\begin{equation}
D = \det|\mathcal{M}|=\det\left|\,
\begin{matrix}
 \phi_1({\bf r}_{1}) & \cdots & \phi_1({\bf r}_{N}) \\
  \,\vdots\hfill&\,\vdots\hfill&\,\vdots\hfill\\
    \phi_{N}({\bf r}_{1}) & \ldots & \phi_{N}({\bf r}_{N})\\
    \end{matrix}
    \right|,
\end{equation}
which ensures the antisymmetric property of a Fermionic wave function upon
exchange of a pair of electrons. The Jastrow factors, which are factorized for
computational efficiency, describe the dynamic correlation, whereas static
correlation is described by the sum of Slater determinants.  

\begin{figure}
%\tiny
  \begin{algorithmic}[1]
    \FOR{$\text{MC generation}=1\cdots M$}
      \FOR{$\text{walker}=1\cdots N_w$}
        \STATE let ${\bf R} = \{{\bf r}_1 \ldots {\bf r}_{N}\}$
        \FOR{$\text{particle}\  i=1 \cdots N$}
           \STATE set ${\bf r}_i^{'} = {\bf r}_i+\delta$
           \STATE let ${\bf R}^{'} = \{{\bf r}_1 \ldots {\bf r}_i^{'} \ldots{\bf r}_{N}\}$
           \STATE \textbf{ratio} $\rho = \Psi_T ({\bf R}^{'})/\Psi_T ({\bf R})$
           \STATE \textbf{derivatives} $\nabla_i \Psi_T, \nabla^2_i\Psi_T$
           \IF{$\vecr \rightarrow \vecr'$ is accepted}
             \STATE update state of a walker
           \ENDIF
        \ENDFOR \COMMENT{particle}
        \STATE \textbf{local energy} $E_L=\hat{H}\Psi_T({\bf R})/\Psi_T({\bf R})$
        \STATE reweight and branch walkers
      \ENDFOR \COMMENT{walker}
      \STATE update $E_T$ and load balance
    \ENDFOR \COMMENT{MC generation}
  \end{algorithmic}
\caption{Pseudocode for diffusion Monte Carlo.\label{alg:DMC}}
\end{figure}

In the diffusion Monte Carlo algorithm (DMC) shown in Fig.~\ref{alg:DMC}, an ensemble of walkers ({\em
population}) is propagated stochastically from generation to generation, where
each walker is represented by $\mathbf{R}$.  In each propagation step, the
walkers are moved through position space by a {\em drift-diffusion process}
(L4-12 of Fig.~\ref{alg:DMC}).  At the end of each step, each walker may
reproduce itself, be killed, or remain unchanged ({\em branching process}),
depending on the value of $E_L$, the local energy, at that point in space.  The
walkers in an ensemble are tightly coupled through a trial energy $E_{T}$ and a
feedback mechanism to keep the average population at the target $10^3-10^5$
walkers.  This leads to a fluctuating population and necessitates shuffling of
walkers among parallel processing units to maintain good load balance in an
appropriate interval (L16 of Fig.~\ref{alg:DMC}).

Most of the computational time is spent on evaluations of ratios (L7), derivatives
for quantum forces (L8) and local energies (L13) in Fig.~\ref{alg:DMC}. The
choice of SPO representation is crucial for QMC efficiency and scalability with
problem sizes.  For a proposed electron move (L5-6) the \code{V}alue, \code{G}radient and
\code{L}aplaican of $N$ SPOs are evaluated at a random particle position
(L7-8) and $N_{ion} N$ \code{V}alues at random positions are evaluated to compute the
pseudopotential contribution with $N_{ion}$ ions (L13).  The cost to compute the
value of a $\phi$ scales linearly with the number of basis function evaluations
which tends to grow with the system size.  This amounts to $\mathcal{O}(N^2)$
cost for each particle move and in total SPO evaluations scale as
$\mathcal{O}(N^3)$ per MC step. 

For this reason, it is efficient to use a localized basis with compact
support.  In particular, 3D tricubic B-splines provide a basis in which only
64 elements are nonzero at any given point in space~\cite{blips4QMC,
einspline}.  The one-dimensional cubic B-spline is given by,
\begin{equation}
f(x) = \sum_{i'=i-1}^{i+2} b^{i'\!,3}(x)\,\,  p_{i'},
\label{eq:SplineFunc}
\end{equation}
where $b^{i}(x)$ are $p_i$ the piecewise cubic polynomial basis functions 
and $i = \text{floor}(\Delta^{-1} x)$ is the index of
the first grid point $\le x$.  Constructing a tensor product in each Cartesian
direction, we can represent a 3D orbital as
\begin{equation}
  \phi_n(x,y,z) = 
  \!\!\!\!\sum_{i'=i-1}^{i+2} \!\! b_x^{i'\!,3}(x) 
  \!\!\!\!\sum_{j'=j-1}^{j+2} \!\! b_y^{j'\!,3}(y) 
  \!\!\!\!\sum_{k'=k-1}^{k+2} \!\! b_z^{k'\!,3}(z) \,\, p_{i', j', k',n}.
\label{eq:TricubicValue}
\end{equation}
This allows the rapid evaluation of each orbital in constant time.
Furthermore, this basis is systematically improvable with a single spacing
parameter, so that accuracy is not compromised.  

The use of 3D tricubic B-splines greatly improves the computational efficiency.
For a typical modest example problem with 32 electrons, the speed up of B-splines
is more than sixfold over an equivalent Plane-Wave (PW) basis set.  The gain
in computation time of B-spline methods becomes increasingly large as the
system size grows.  On the downside, this computational efficiency comes at
the expense of increased memory use, which is easily overcome by the large
aggregate memory available per node through OpenMP/MPI hybrid QMC.

\subsection{Einspline library}\label{sec:einspline}
As the most performance-critical component in QMCPACK, 3D B-splines orbitals
have been extensively optimized over the years~\cite{einspline}.  Key improvements include
\begin{itemize}
\item The memory layout of the B-splines coefficients, $b$ in
Eq.~\ref{eq:TricubicValue}, is transformed from \code{b[N][Nx][Ny][Nz]} (AoS)
to \code{b[Nx][Ny][Nz][N]} (SoA) to compute $N$ orbitals at a random position. 
\item Multiple algorithms using loop transformations and unrolling have been developed.
\item Improved algorithms are implemented in
intrinsics, SSE/-SSE2 on x86 systems and QPX on BG/Q~\cite{YeSC15}.  
\item The B-spline coefficients are stored in a single-precision (SP)
container and SPOs are computed in SP ~\cite{qmcpackGPU}. 
\end{itemize}
The QMCPACK build system allows selecting optimal algorithms and implementations
at the compiler time.  The baseline of this work uses the latest optimized
implementations in C/C++ in the official QMCPACK
distribution~\cite{qmcpack,YeSC15}.

%Being one of the most time consuming parts in QMCPACK, implementation of
%B-Spline operations have been optimized over past many years. These include
%modifying the data layout of read only coefficient array to have spline
%dimension as inner most, algorithm modification by changing order of loops,
%writing intrinsics for SSE and on Blue-gene Q etc. In this publication, we
%evaluated various algorithms and find Ye's implementation the best and take it
%as our baseline [ref for SC15 poster] to build our improvements on top of that.



